A Distributed Multi-Vehicle Coordination Algorithm for Navigation in Tight Environments

This work presents a distributed method for multi-vehicle coordination based on nonlinear model predictive control (NMPC) and dual decomposition. Our approach allows the vehicles to coordinate in tight spaces (e.g., busy highway lanes or parking lots) by using a polytopic description of each vehicle's shape and formulating collision avoidance as a dual optimization problem. Our method accommodates heterogeneous teams of vehicles (i.e., vehicles with different polytopic shapes and dynamic models can be part of the same team). Our method allows the vehicles to share their intentions in a distributed fashion without relying on a central coordinator and efficiently provides collision-free trajectories for the vehicles. In addition, our method decouples the individual-vehicles' trajectory optimization from their collision-avoidance objectives enhancing the scalability of the method and allowing one to exploit parallel hardware architectures. All these features are particularly important for vehicular applications, where the systems operate at high-frequency rates in dynamic environments. To validate our method, we apply it in a vehicular application, that is, the autonomous lane-merging of a team of connected vehicles to form a platoon. We compare our design with the centralized NMPC design to show the computational benefits of the proposed distributed algorithm.

==> Extra.tex <==
\begin{equation}\label{eq:MPC_formulation_reformulated}
\begin{aligned}
% & \underset{{u^i(.|t)},\lambda_{ij}(.|t), \mu_{ij}(.|t), s_{ij}(.|t)}{\text{minimize}}
& \min_{\substack{\mathbf{u}^i(\cdot|t),\ \mathbf{\lambda}_{ij}(\cdot|t),\\ \mathbf{\mu}_{ij}(\cdot|t),\ \mathbf{s}_{ij}(\cdot|t)}}
& & \eqref{eq:total_cost} \\
&\textrm{subject to} & &
\eqref{eq:dynamic_constraint},\eqref{eq:initial_cond}, \eqref{eq:states_bound}, \eqref{eq:input_bound},\\
& & & \big(-\mathbf{b}_{i}(\mathbf{z}^{i}(k|t))^{\top} \mathbf{\lambda}_{ij}(k|t) \\
& & & - \mathbf{b}_{j}(\mathbf{z}^{j}(k|t))^{\top} \mathbf{\mu}_{ij}(k|t)\big) \geq d_\text{min},\\
& & & \mathbf{A}_{i}(\mathbf{z}^{i}(k|t))^{\top} \mathbf{\lambda}_{ij}(k|t) + \mathbf{s}_{ij}(k|t) = 0,\\
& & & \mathbf{A}_{j}(\mathbf{z}^{j}(k|t))^{\top} \mathbf{\mu}_{ij}(k|t) - \mathbf{s}_{ij}(k|t) = 0,\\
& & & \|{\mathbf{s}_{ij}(k|t)}\| \leq 1, -\mathbf{\lambda}_{ij}(k|t) \leq 0, \\
& & & -\mathbf{\mu}_{ij}(k|t) \leq 0, \text{for all } i \in \mathcal{V},\ j \in \mathcal{N}_i,\\
\end{aligned} \end{equation}


mpc module formulation
\begin{subequations}\label{eq:MPC_module}
\begin{align}
& \min_{\substack{u^i(\cdot|t)}}
& &\nonumber{\sum_{k=t}^{t+N}Q||z^{i}(k|t)-z^{i}_\textrm{Ref}(k|t)||^2_2} \\
\label{eq:input_cost}
& & &+ \sum_{k=t}^{t+N-1}R_1||u^{i}(k|t)||^2_2 + R_2||\Delta u^{i}(k|t)||^2_2\\
&\textrm{subject to} & &
\eqref{eq:dynamic_constraint},\eqref{eq:initial_cond}, \eqref{eq:states_bound}, \eqref{eq:input_bound},\\
& & & \big(-b_{i}(z^{i}(k|t))^{\top} \lambda_{ij} - b_{j}^{\top} \lambda_{ji}\big) \geq d_\text{min},\\
& & & A_{i}(z^{i}(k|t))^{\top} \lambda_{ij} + s_{ij} = 0,\\
& & & \text{for all } i \in \mathcal{V},\ j \in \mathcal{N}_i,
\end{align} \end{subequations}

\begin{itemize}
    \item While reading formation-control-rectangular-agents.pdf they claim they are using rectangular-shape modeling that can be extended to more vertices if needed and use a potential-field-based approach to design the formation control law to enable agents to avoid collision with each other and the obstacles. Their approach, however, seems to only consider simple robot dynamics and rely only on potential field functions. Our approach can handle more complex models and potential fields functions can also be accommodated by the MPC framework (for example we used them for our car and Jackal robot to increase clearance from the obstacles). In addition, based on my experience with potential field functions it is not possible to ensure exact collision avoidance in tight spaces. Can we show a simulation in which one of the car is actually static (as a static obstacle) and the other cars have to overtake it? In addition, it would be great to show a scenario with a car not part of the formation (moving at constant speed) that is overtaken by the other cars. To simulate this scenario you can consider one of the cars having adot = 0 and see what happens. 
    \item Can you double-check the paper references/good-for-references-cooperative-collision-avoidance-for-nonholonic-robots.pdf? I think it is good for references, but I am having a hard time to understand what they do (I would ask Javier directly but he is on sick leave till the end of the month). First they use motion primitives that we do not use. They specify that they can include robot dynamics, but I think they are only used to generate the motion primitives. Then, for collision avoidance, they do use a polytopic representation of the obstacles (if I understand correctly) transformed in velocity space that it is either linearized or a mixed integer programming problem. In our case, we do not need linearization because we rely on duality theory right? In addition, the robots themselves are always approximated with circles right?
\end{itemize}
\roya{About item 2: I read the Javier paper, they assume the robot is locally non-rotating during the time horizon of the local planner. Yes, my understanding is that they don't include the dynamics, they use it to generate motion primitives. About linearization in velocity space, yes that is correct that we don't use linearization because we rely on duality. One thing that is interesting is that they say one drawback of the linearization is that the solution space reduces.}
\paragraph{Related work}
\laura{I am collecting some references in the folder "references". I found a nice survey paper (survey-paper-2013.pdf) and a more recent paper that has a nice structure for our related work section (formation-control-rectangular-agents.pdf). }


\laura{does the method applies just to 2D planning or also 3D (for example drones)? If the method applies also to 3D planning we should emphasize it.}
\roya{Yes, the method can be applied to 3D platooning for drones as well.}\laura{Then, this is also a big plus compared to other methods.}


\footnote{\laura{It might be better to have a separate section in which we define the sets of static and dynamic obstacles and the conditions for collision avoidance. You can look at Section II of this paper to have an idea of what I mean: \url{http://www.alonsomora.com/docs/19-zhu-icra.pdf}} \roya{This paper is interesting! I need some time to go over it.}\laura{It is just to give you an idea how we structured the preliminary section. It could help us save some space :)}}

\footnote{\laura{Can you add the definition of the polytopic set? It might not be straightforward for a robotics audience.} \roya{just added}}

\footnote{\laura{Can you provide more details? E.g., is it RRT, $A^*$?}\roya{It is just a simple integration forward in time. I am gonna talk to you about this}}


\footnote{\laura{What is the difference between $\mathcal{O}$ and $\mathcal S$?.}\roya{$\mathcal{O}$ is just one static obstacle but $\mathcal S$ is the set of all static obstacles including $\mathcal{O}$}}

The set of neighbors of robot $i$ is denoted as $\mathcal{N}_i$ is the set of all the robots within the neighborhood of $i$th robot and is defined as $\mathcal{N}_i = \mathcal{V} \setminus i$. 

where $\mathbf{z}(k)$ represents the robot state at $k$th time step, $\mathcal{P}(\mathbf{z}(k))$ is the robot occupied region as a function of the state $\mathbf{z}(k)$

\item \emph{Polytopic Description of Robot Pose:} Robot pose or the region occupied by the robot can be described as a convex set defined by a polytope $\mathcal{P}$. Polytopes are described as the intersection of a set of half-spaces and are defined as a set of linear inequalities. The polytopic representation is a function of the state of the robot $z(t)$ at current time $t$. The initial pose of the robot is represented as $\mathcal{P}_{o}$. As the robot travels, $\mathcal{P}_{o}$ undergoes affine transformations including rotation and translation. Hence $\mathcal{P}(\mathbf{z}(t)) = \mathbf{R(\mathbf{z}(t))}\mathcal{P}_{o} + \mathbf{t(\mathbf{z}(t))}$, where $\mathbf{R}:\mathbb{R}^{n_{z}} \rightarrow \mathbb{R}^{n\times n}$ is an orthogonal rotation matrix and $\mathbf{t}:\mathbb{R}^{n_{z}} \rightarrow \mathbb{R}^{n}$ is the translation vector, where $n_z$ is the dimension of the robot state $z$ and $n$ is dimension of the space which is 2 for 2D- and 3 for 3D planning.


\begin{equation}\label{eq:individual_cost}
\begin{aligned}
J^i(\mathbf{z}^{i},\mathbf{u}^{i}) &= \sum_{k=t}^{t+N}||\mathbf{Q}(\mathbf{z}^{i}(k|t)-\mathbf{z}^{i}_\textrm{Ref}(k|t))||^2_2 \\
&+ \sum_{k=t}^{t+N-1}||\mathbf{R_1}(\mathbf{u}^{i}(k|t))||^2_2 + ||\mathbf{R_2}(\Delta \mathbf{u}^{i}(k|t))||^2_2.\\
\end{aligned}
\end{equation}

generic stage cost

 The reference trajectory obtained from the high-level planner is denoted as $\mathbf{z^{i}}_\text{Ref}$ 
 
 A global (high-level) motion planner like A* or RRT* generates that global tentative trajectory that can collide with obstacles. In local (low-level) an MPC controller plans collision-free motions. 
 
 
 % Comments August 28
 I rewrote the abstract and the first part of the introduction (I Still need to finalize the related work) to shorten them a bit and address also George's concerns. I also moved figure 1 on the first page. Somehow a lot of robotics papers have a figure there to explain the approach or show the testing platform. I started to finalize the references in the first part of the introduction for now. In addition, I was thinking whether Fig. 2 is needed. 
 
 % Comments August 29
 I think we could modify the title with something like: "A Distributed Multi-Robot Coordination Algorithm for Navigation in Tight Environments". What do you think?
 
 Also I added extra references in the related work. Please feel free to add more (I saw that George has a nice related work section in his paper).
 
 I modified Figure 1. Let me know what you think. 
 
 I modified Figure 2. Let me know what you think. I wanted to emphasize that the calculations are in parallel and each robots perform them locally. I also wanted to show how they occur over time. 
 
 Experiments: how do you compute the computation time? Usually to measure time in a more accurate way I run the same experiment 11 times and then I take the mean, median, and max of all the 11 runs. Also can we say that the results were obtained for 2,3, 4 vehicles for different initial configurations? We need to comment on the tuning parameters and how they can affect the performance (e.g., deadlocks). Concerning the implementation, is it the solver running in C or also the solver is in MATLAB? 
 
 Please check the notation. At the moment you are using the superscript for the state trajectories, while the subscript for the dual variables. I will put either all as a subscript or all as a superscript. In addition, there are some superscripts/subscripts in italic and other in bold. 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 \laura{The optimal solution is $\mathbf{u}^*(t) = [u^*(k|t),...,u^*(k+N-1|t)]$, and the receding horizon control law is obtained by applying the first control input $u_{\textrm{MPC}}(t) = u^*(t|t).$\footnote{\laura{I think also this sentence is not needed, since we have it defined in the preliminaries.}}}
 
 \laura{$\boldsymbol{\lambda}_{ij}(\cdot|t)$, $\boldsymbol{\lambda}_{ji}(\cdot|t)$ and $\mathbf{s}_{ij}(\cdot|t)$ represent the sequence of dual variables over the MPC horizon $N$. For example, $\boldsymbol{\lambda}_{ij}(\cdot|t) = [\boldsymbol{\lambda}_{ij}(t|t),...,\boldsymbol{\lambda}_{ij}(t+N|t)]$.\footnote{\laura{I would remove this sentence.}}}
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  9/4/2019
 1) \footnote{\laura{Here you are specifying the the superscript $\mathbf i$ indicates the robot, while later you always use the superscript $\mathbf i$.}} \roya{ is it clear now? or you want them to have the same superscript or subscript?}
 
 2) \footnote{\laura{Can we remove this last sentence? It is mentioned again later for dynamic obstacles.}}:
 \roya{Shouldn't I represent the definition for neighbor set?
 I added this instead: $\mathcal{N}_i$ and represents all the robots that are in the communication range of Robot $i$.}
 
 3) \footnote{\laura{Is this correct? I think the Rotation matrix depends on the orientation of the robot, while $\mathcal P$ depends on the position, right? Or do we make the assumption that $\mathbf R$ does not vary over time?}\roya{polytope p is representation of both heading and position. It is not just position. Also, yes rotation R is a function of heading angle and translation t is a function of position (x,y)}. Also rotation is time-varying, it is nor assumed to be constant.}
 
 4) \footnote{\laura{$\mathbf t$ might be confusing, given that we are using $t$ also to indicate time. It is not a big problem, but if you have a better notation in mind please update it.} \roya{I changed it to t_r. Let me know if you have any other suggestion}}
 
 5)\footnote{\laura{Do we really need that $\mathcal{O}^{r}$ is a polytope?I think the definition of collision avoidance you use could work with any static obstacle shape right?}\roya{In this paper everything should be polytope. But the method can be generalized to other convex shapes in the future.}}
 
 6)\footnote{\laura{I think that if we have \eqref{eq:initial_cond} in the problem formulation, there is no need of using the notation $\mathbf{z}^i(k|t)$, because it is clear from the initial state that \eqref{eq:dynamic_constraint} are the predictions based on the initial condition at time $t$.}\roya{Let's keep it this way, I'll talk to you about this.}}
 
 7)\laura{\footnote{\laura{From the current formulation of the dual problem it is hard to understand where $d_\min$ plays a role. Can you just reformulate the minimum distance in primal and dual form with $d_\min$ rather than 0? Otherwise please provide more details to explain the connection with $d_\min$}\roya{$d_\min$ is already included in the constraint (5a) in the MPC module. So $z$ variables in NMPC module are selected in such a way to respect $d_\min$}}}
 
 8)\footnote{\laura{Do you think we can formulate this equivalence as a lemma or a theorem? Like \eqref{eq:dual} is equivalent to the fealibility problem XXX. Then, the proof can be a sketch or a reference to~\cite{Zhang2018}.}\roya{feasibility problem is actually a relaxation of \eqref{eq:dual}. I can also confirm with Geroge, but I think actually they are not equivalent.}}
 
 9) \laura{\footnote{\laura{I changed algorithm~\ref{alg_coordination}. I wanted to give an idea of what each robot is doing at every step and that they do it in parallel. I also reduced the font size of the algorithm to gain more space. Please let me know what you think. If it is more clear now what each robot is doing we could remove figure 2.}\roya{yes, if we remove figure 2., we can include it in the video. Let's talk about parallelization}}}
 
 % September 6th
 I suggest to remove the superscript $i$ in the description of the model of the vehicles in the Sec V-A adding that we omit the superscript when it is clear from the context. I think it improves readability. If you want you can restore the previous version (it is just commented out). If you do so, you need to add some superscripts (for example when describing the polytopes of each vehicle, the length and width of the vehicle, etc).
 
 Equation (3). Check if it is better written in this way. I found it a bit strange while reading the section again compared with the other problem definitions.
 
 I left all the main new parts in purple so you can have a look at them. I have been looking for relevant reference to add in the related work. I wanted to add an approach that explicitly mentioned separating hyperplanes to state the difference with our method. Let me know what you think and feel free to re-phrase it or add more references.
 %%%%%%%%%%%%%%%%%%%%%%%%%%
  % November 13th
 Goal: By assuming that centralized formulation (4) has a feasible solution, we want to show that the distributed NMPC formulation (5) has a feasible solution as well, under some condition. 

Assume a feasible solution of problem (4) is $(\mathbf{u}^*,\mathbf{z}^*)$ and if we consider boundary condition for the constraint (4a) we have:
$-\mathbf{b}^i(\mathbf{z}^i)^{\top} \boldsymbol{\lambda}_{ij}- \mathbf{b}^j(\mathbf{z}^{j})^{\top} \boldsymbol{\lambda}_{ji} = d_\text{min}$ and we can solve the equation to find a closed-form expression for $\boldsymbol{\lambda_{ij}}$. Also using constraints (4b) and (4c) we have: 
$\mathbf{A}^i(\mathbf{z}^i)^{\top} \boldsymbol{\lambda}_{ij}\! = -\mathbf{A}^j(\mathbf{z}^j)^{\top} \boldsymbol{\lambda}_{ji}$. Thus by substituting $\lambda_{ji}$ in the above equation we get:
$-\mathbf{b}^i(\mathbf{z}^i)^{\top} \boldsymbol{\lambda}_{ij}- \mathbf{b}^j(\mathbf{z}^{j})^{\top} (-\mathbf{A}^j(\mathbf{z}^j)^{-\top}\mathbf{A}^i(\mathbf{z}^i)\boldsymbol{\lambda}_{ij}) = d_\text{min}.$ If we solve for $\boldsymbol{\lambda_{ij}}$, we have:
\begin{equation}
    (\mathbf{A}^i {\mathbf{A}^j}^{-1}\mathbf{b}^j - \mathbf{b}^i)^{\top} \boldsymbol{\lambda}_{ij} = d_\text{min}
\end{equation}
This equation is a linear program which can be solved by solving another minimization under the constraint that $\boldsymbol{\lambda_{ij}}$ is non-negative, and also $||\mathbf{A}^i\boldsymbol{\lambda}_{ij}|| \leq 1$. Therefore, we cannot find an expression for feasible $\boldsymbol{\lambda_{ij}}$, obtained by centralized formulation (4). 

Now let's assume that we already have obtained a feasible solution for $\boldsymbol{\lambda_{ij}^c}$ from centralized formulation (4). Also assume that the solution of distributed formulation (5) is always a linear combination of the centralized formulation (4) and a positive quantity $\boldsymbol{\lambda_{ij}^{\text{delay}}}$, as 
\begin{equation}
    \boldsymbol{\lambda}_{ij}^d = \boldsymbol{\lambda}_{ij}^c + \boldsymbol{\lambda}_{ij}^{\text{delay}}
\end{equation}
If we substitute $\boldsymbol{\lambda}_{ij}^d$ in distributed formulation equation (5a) we get:
\begin{equation}
    -(\mathbf{b}^i)^{\top} (\boldsymbol{\lambda}_{ij}^c + \boldsymbol{\lambda}_{ij}^{\text{delay}})- (\mathbf{b}^j)^{\top}(\boldsymbol{\lambda}_{ji}^c + \boldsymbol{\lambda}_{ji}^{\text{delay}}) \geq d_\text{min}
\end{equation}
Since $-(\mathbf{b}^i)^{\top} \boldsymbol{\lambda}_{ij}^c-(\mathbf{b}^j)^{\top} \boldsymbol{\lambda}_{ji}^c = d_\text{min}$, thus we get:
\begin{equation}
    -(\mathbf{b}^i)^{\top} (\boldsymbol{\lambda}_{ij}^{\text{delay}})- (\mathbf{b}^j)^{\top}(\boldsymbol{\lambda}_{ji}^{\text{delay}}) \geq 0
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%December 5:
We know $||(\mathbf{A}^{\top})^{\dagger}||_{2} = \sigma_\text{max}$, so 
\begin{equation}
    ||\big(\boldsymbol{\lambda}_{ij}\big)_\mathbf{c} - \big(\boldsymbol{\lambda}_{ij}\big)_\mathbf{d}|| \leq  \big(\sigma_\text{max}\big)_\mathbf{c} + \big(\sigma_\text{max}\big)_\mathbf{d}.
\end{equation}

\begin{equation}
\begin{aligned}
    ||\big(\boldsymbol{s}_{ij}\big)_\mathbf{c}\! - \big(\boldsymbol{s}_{ij}\big)_\mathbf{d}||
    = ||\big(\mathbf{A}^i(\mathbf{z}^i)^{\top} \boldsymbol{\lambda}_{ij}\big)_\mathbf{c}\! - \big(\mathbf{A}^i(\mathbf{z}^i)^{\top} \boldsymbol{\lambda}_{ij}\big)_\mathbf{d}|| & \leq\\ ||\big(\mathbf{A}^i(\mathbf{z}^i)^{\top} \boldsymbol{\lambda}_{ij}\big)_\mathbf{c}||\! + ||\big(\mathbf{A}^i(\mathbf{z}^i)^{\top} \boldsymbol{\lambda}_{ij}\big)_\mathbf{d}||
    \end{aligned}
\end{equation}

%%%%%%%%%%%%%%%%%%%%
December 13:
Since finding the Euclidean distance for $\mathbf{z}$ values obtained by centralized and distributed approaches is hard due to nonlinear constraints of dynamics and collision avoidance, we establish an upper-bound on the difference of actual minimum distance obtained by the two methods. 
The distance between robot $i$ and robot $j$ is defined as $-{\mathbf{b}^{i}}^{\top} \boldsymbol{\lambda}_{ij} - {\mathbf{b}^{j}}^{\top} \boldsymbol{\lambda}_{ji}$. 

\begin{equation}
\begin{aligned}
    &||\big(-{\mathbf{b}^{i}}^{\top} \boldsymbol{\lambda}_{ij} - {\mathbf{b}^{j}}^{\top} \boldsymbol{\lambda}_{ji}\big)_{c} - \big(-{\mathbf{b}^{i}}^{\top} \boldsymbol{\lambda}_{ij} - {\mathbf{b}^{j}}^{\top} \boldsymbol{\lambda}_{ji}\big)_{d}||\leq\\
    &||\big(-{\mathbf{b}^{i}}^{\top} \boldsymbol{\lambda}_{ij} - {\mathbf{b}^{j}}^{\top} \boldsymbol{\lambda}_{ji}\big)_{c}|| + ||\big(-{\mathbf{b}^{i}}^{\top} \boldsymbol{\lambda}_{ij} - {\mathbf{b}^{j}}^{\top} \boldsymbol{\lambda}_{ji}\big)_{d}||\leq\\
    &||\big(-{\mathbf{b}^{i}}^{\top} \boldsymbol{\lambda}_{ij}\big)_{c}||+ ||\big({\mathbf{b}^{j}}^{\top} \boldsymbol{\lambda}_{ji}\big)_{c}|| +\\ &||\big(-{\mathbf{b}^{i}}^{\top} \boldsymbol{\lambda}_{ij}\big)_{d}||+ ||\big({\mathbf{b}^{j}}^{\top} \boldsymbol{\lambda}_{ji}\big)_{d}||\leq\\
    &||\big({\mathbf{b}^{i}}^{\top}\big)_{c}||\ ||\big(\boldsymbol{\lambda}_{ij}\big)_{c}||+ ||\big({\mathbf{b}^{j}}^{\top}\big)_{c}||\ ||\big(\boldsymbol{\lambda}_{ji}\big)_{c}||\\
    &||\big({\mathbf{b}^{i}}^{\top}\big)_{d}||\ ||\big(\boldsymbol{\lambda}_{ij}\big)_{d}||+ ||\big({\mathbf{b}^{j}}^{\top}\big)_{d}||\ ||\big(\boldsymbol{\lambda}_{ji}\big)_{d}||\leq\\
    &||\big({\mathbf{b}^{i}}\big)_{c}||\ + ||\big({\mathbf{b}^{j}}\big)_{c}||+
    ||\big({\mathbf{b}^{i}}\big)_{d}||\ + ||\big({\mathbf{b}^{j}}\big)_{d}||
    
\end{aligned}
\end{equation}

Since in our application, $\mathbf{b}(\mathbf{z}(t)) = [
h/2,w/2,h/2,w/2]^\top$ $+ \mathbf{A}(\mathbf{z}(t))[
x(t),
y(t)
]^{\top}$, then by taking the norm of both sides we have
\begin{equation}
\begin{aligned}
||\mathbf{b}(\mathbf{z}(t))|| &= ||[
h/2,w/2,h/2,w/2]^\top||+\\
&||\mathbf{A}(\mathbf{z}(t))[
x(t),
y(t)
]^{\top}|| \leq\\
& ||[
h/2,w/2,h/2,w/2]^\top|| +\\ &||\mathbf{A}(\mathbf{z}(t))||_{\mathbf{F}}\ ||[
x(t),
y(t)
]^{\top}||,
\end{aligned}
\end{equation}
since $||\mathbf{A}(\mathbf{z}(t))||_{\mathbf{F}} = 1$ we have
\begin{equation}
\begin{aligned}
||\mathbf{b}(\mathbf{z}(t))|| \leq 
& ||[
h/2,w/2,h/2,w/2]^\top|| + ||[
x(t),
y(t)
]^{\top}||,
\end{aligned}
\end{equation}
%%%%%%%%%%%%%%%
\begin{equation}
\begin{aligned}
&||\mathbf{ b}^i(\mathbf{ z}^i(t))-\bar{\mathbf{b}}^i(\bar{\mathbf{z}}^i(t-1))||\\
&= \mathbf{A}(\psi(t))\begin{bmatrix}
x(t)\\
y(t)
\end{bmatrix}-\mathbf{A}(\bar{\psi}(t-1))\begin{bmatrix}
\bar{x}(t-1)\\
\bar{y}(t-1)
\end{bmatrix}\\
&\mathbf{A}(\psi(t))\begin{bmatrix}
\bar{x}(t-1)+\Delta t\ v(t) \cos{\psi(t)}\\
\bar{y}(t-1)+\Delta t\ v(t) \sin{\psi(t)}
\end{bmatrix}\\
&-\mathbf{A}(\bar{\psi}(t-1))\begin{bmatrix}
\bar{x}(t-1)\\
\bar{y}(t-1)
\end{bmatrix}\\
&= \sqrt{2}\bigg(\big(\bar{x}(t-1)\big(\cos{\psi(t)}-\cos{\bar{\psi}(t-1)})\\
&-\bar{y}(t-1)\big(\sin{\psi(t)}-\sin{\bar{\psi}(t-1)}\big)\\
&+ \Delta t\ v(t) \cos{2\psi(t)}\big)^2\\
&\big(\bar{y}(t-1)\big(\cos{\psi(t)}-\cos{\bar{\psi}(t-1)})\\
&-\bar{x}(t-1)\big(\sin{\psi(t)}-\sin{\bar{\psi}(t-1)}\big)\\
&+ \Delta t\ v(t) \sin{2\psi(t)}\big)^2\bigg)^\frac{1}{2}
\end{aligned}
\end{equation}
 
By defining the acceptable error in between predicted and realized trajectories for $x$,$y$ and $\psi$ values, we can define a threshold for the upper-bound and include the upper-bound \eqref{upper_bound} in the NMPC formulation \eqref{eq:MPC_module} to bound the prediction error in the distributed problem. The maximum error on $x$, $y$ and $\psi$ are denoted as $e_x$, $e_y$ and $e_{\psi}$, respectively and defined as
\begin{equation}\label{error_eq}
\begin{aligned}
    e_x &= x(t) - \bar{x}(t-1)\\
    e_y &= y(t) - \bar{y}(t-1)\\
    e_{\psi} &= \psi(t) - \bar{\psi}(t-1)
\end{aligned}
\end{equation}
On the other hand Euler discretization on dynamic model and substituting \eqref{error_eq} in them we have
\begin{equation}
\begin{aligned}
    e_x &= x(t)-\bar{x}(t-1) = \Delta t\ v(t) \cos{\psi(t)}\\
    e_y &= y(t)-\bar{y}(t-1) = \Delta t\ v(t) \sin{\psi(t)}
\end{aligned}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% Feb 4th

So the idea would be the following (if I understand correctly):
1) add to the NMPC module, Eq. 27 (maybe as a term in the cost?) to limit the increment between two iterations; 2) select the bounds on the increments ($e_x, e_y, $ and $e_\psi$) to get a desired value of $\alpha$ and limit the upper bound we computed to a reasonable value. Is this correct? I think this idea is nice and allows the algorithm to quantify on line the error. It is a sort of adaptive MPC strategy. I am thinking whether we could anticipate for such an error in the CA module (Eq. 6). It might be nice if the lambda values could already account for this errors in order to reduce the upper bound. Did you have any idea about it? 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Also to further improve the computation time, the nonlinear dynamics can be linearized around the trajectory computed by the previous step of MPC. Then the NMPC module will be transformed to a convex-QP problem and can be solved faster then the current nonlinear formulation. Another future work will be generalization of modeling the robot shape and extending it to other shapes such as ellipsoids and in general convex sets, using the same dual formulation and decomposition. 
Our aim is to generalize the approach to general convex sets to accommodate within a uniform dual framework any robot shape (e.g., ellipsoids, ellipses and circles). 
Finally, our current approach models robots using polytopes. 

%%%%%%%
Abstract Copy
This work presents a distributed nonlinear model predictive control (NMPC) approach for multi-robot coordination. Our method allows the robots to coordinate in tight spaces (e.g., highway lanes, canals) by using a polytopic description of each robot's shape and formulating the collision avoidance problem in a dual optimization framework. Our method accommodates heterogeneous teams of robots (i.e., robots with different polytopic shapes and dynamic models can be part of the same team) and can be used to avoid collisions in $n$-dimensional spaces. Starting from a centralized implementation of the NMPC problem, we show how to exploit the problem structure to allow the robots to cooperate---communicating their intentions to the neighbors---and compute collision-free paths in a fully distributed way. By relying on a bi-level optimization strategy, our design decouples the optimization of the robot states and of the collision-avoidance variables to make the overall coordination strategy more scalable and efficient (in terms of computation time). Compared to a centralized design, the proposed decomposition introduces a local prediction error that could lead to more conservative local trajectories. Nevertheless, we show that this error is bounded and can be accounted for in the local NMPC problems. Finally, we validate our method for an autonomous driving application, that is, the autonomous navigation of a platoon of connected vehicles on public roads. We compare our design with the initial centralized NMPC design to show the computational benefits of our distributed algorithm. %Nevertheless, the proposed approach is general and can be applied to different applications and robot models.
Videos and software can be found online here...

%%
The robots communicates with its neighbors within the communication radius. The robots have a limited communication radius so that the number of robots we will have to coordinate is somehow limit

we can use this insight to reformulate the dual problem as the following feasibility problem 
 
keep it more concise here you could think using directly the symbols, e.g., a$\in[-4,\, 4]$ m/s$^2$


Note that we show simulations for up to four vehicles to be able to perform parallel computing on the available four-core CPU and be able to compare with the centralized implementation of our design.

%%%%%%%%%%%%%%
Discrepancy \\
The distributed NMPC \eqref{eq:MPC_module} returns a suboptimal solution compared to the centralized NMPC \eqref{eq:MPC_centralized}, due to two main sources of discrepancy:\\
\emph{a) Bi-level optimization scheme.}
The distributed Algorithm \ref{alg_coordination} is a multi-level optimization with NMPC module \eqref{eq:MPC_module} as the upper-level optimization and the CA module \eqref{eq:collision_module} as the lower-level optimization. Solving lower-level CA module and substituting its solution in the upper-level NMPC module further restricts the constraints \eqref{NMPC_dmin}-\eqref{distributed_sij}, since the dual variables are kept fixed (i.e., the optimizer has less degree of freedom in the computation of the local trajectories). In contrast, in the centralized NMPC \eqref{eq:MPC_centralized}, the equivalent constraints \eqref{eq:coupling_constraint}-\eqref{eq:coupling_sep_hyp_neg} are relaxed compared to the constraints \eqref{NMPC_dmin}-\eqref{distributed_sij}, since the dual variables are decision variables of the centralized problem.\\
\emph{b) Trajectory prediction error.}
In general for inherently decoupled systems, the source of discrepancy between centralized and distributed approaches is caused by communication delay (or trajectory prediction error among neighbor robots). As the communication delay increases, the solution of distributed problem differs from the optimal centralized solution. So for fast enough communication rate, both problems yield the same solution. In this paper, our problem is a coupled problem in which we break the coupling by exploiting the dual structure using bi-level optimization.
%%%%%%%%%%%%
According to constraint \eqref{eq:coupling_sep_hyp_pos}, we have
\begin{equation}
    \mathbf{A}^i(\mathbf{z}^i)^{\top} \boldsymbol{\lambda}_{ij} + \mathbf{s_{ij}} = 0,
\end{equation}
so,
\begin{equation}
    \boldsymbol{\lambda}_{ij} = - (\mathbf{A}^i(\mathbf{z}^i)^{\top})^{\dagger} \mathbf{s_{ij}},
\end{equation}
where $\mathbf{A}^{\dagger}$ is $(\mathbf{A}^{\top}\mathbf{A})^{-1}\mathbf{A}^{\top}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Disadvantage
The disadvantage is that the local NMPC modules have less degrees of freedom to compute the individual trajectories (they cannot optimize the collision-avoidance variables) leading to more conservative trajectories. In addition, the communication delay among the robots can generate a prediction error that could compromise the safety of the robot coordination.


\begin{algorithm}[t]
\caption{\small Distributed Coordination Algorithm}\label{alg_coordination}
    \begin{algorithmic}[1]
        \State Initialize $[\mathbf{s}_{ij}(0),...,\!\mathbf{s}_{ij}(N)],$ $[\boldsymbol{\lambda}_{ij}(0),...,\boldsymbol{\lambda}_{ij}(N)],$ $[\boldsymbol{\lambda}_{ji}(0),...,\boldsymbol{\lambda}_{ji}(N)]$, $\forall i,j \in \mathcal{N}$  and $i\neq j.$
        \For { $t=0,1,..., \infty$} 
        \ForAll {Robot $i$, $i\in \mathcal V$} \Comment{in parallel}
          \State {Solve NMPC Optimization} %: $[\mathbf{z}^i(1),...,\mathbf{z}^i(N)]$}.
        \State {Compute the shifted state trajectory $[\mathbf{z}^i(1),...,\mathbf{z}^i(N),\mathbf{z}^i(N)]$.}
        \State  {Compute the associated polytopic sets: $[\mathbf{A}^i(1),...,$ \hphantom{zzzzzzz}$\mathbf{A}^i(N),$ $\mathbf{A}^i(N)]$, $[\mathbf{b}^i(1),$..., $\mathbf{b}^i(N),$ $\mathbf{b}^i(N)].$}
        \State {Communicate to Robot $j$ ($\forall j \in \mathcal N_i$) the polytopic sets.}
        \State {Solve Collision Avoidance Optimization for each $j \in \mathcal{N}_i$.}
        %:        $[\mathbf{s}_{ij}(1),...,\mathbf{s}_{ij}(N)]$, $[\boldsymbol{\lambda}_{ij}(1),...,\boldsymbol{\lambda}_{ij}(N)],$ $[\boldsymbol{\lambda}_{ji}(1),...,\boldsymbol{\lambda}_{ji}(N)].$ 
        \State {Apply $\mathbf{u}_{\text{MPC}}^{i}$ to move forward.}
        \EndFor
        \EndFor
    \end{algorithmic}
\end{algorithm}

==> SEC6.tex <==
\section{Prediction Error Bound}
\label{SEC6}
In this section we focus on the discrepancy between distributed and centralized approaches caused by trajectory prediction error. In the centralized approach \eqref{eq:MPC_formulation}, since the coordinator chooses the optimal action for all the vehicles simultaneously, the approach does not rely on the open-loop trajectories of the neighbor vehicles (no communication is involved). However, in the distributed problem \eqref{eq:MPC_optimization}, each vehicle optimizes its own action based on the communicated information about the predicted (open-loop) trajectories of other vehicles. In this section, we quantify the trajectory prediction error and establish an upper bound on this error. To help the discussion, we consider a simple simulation scenario and present all the results for this scenario. In this scenario, two cars, namely, car $i$ and car $j$, are moving in the same direction using two different lanes when car $i$ decides to overtake and merge into car $j$'s lane, as shown in \figref{fig:scenario_example}, (for more details on the model and formulation refer to Sec.~\ref{subsec:platoon_formation}). 

Consider the open-loop trajectory of vehicle $i$ predicted by vehicle $i$ as $\boldsymbol{\tau}^i_{pi}(t) = [\mathbf{z}^i(0|t),\mathbf{z}^i(1|t),\dotsc,\mathbf{z}^i(N|t)]$ and the shifted and augmented open-loop trajectory of vehicle $i$ predicted by vehicle $j$ as $\boldsymbol{\bar \tau}^i_{pj}(t-1) = [\mathbf{\bar z}^i(1|t-1),\mathbf{\bar z}^i(2|t-1),\dotsc,\mathbf{\bar z}^i(N|t-1), \mathbf{\bar z}^i(N|t-1)]$, (the trajectory is shifted one step forward in time and augmented with the same last value). The subscript $pi$ means predicted by vehicle $i$ and similarly $pj$ means predicted by vehicle $j$. Also $\boldsymbol{ \tau}^j_{pj}(t)$ represents trajectory of vehicle $j$ predicted by $j$ at current time step $t$ and $\boldsymbol{\bar \tau}^i_{pj}(t-1)$ denotes the trajectory of vehicle $i$ predicted by vehicle $j$ at the previous time step $t-1$. 
 
The prediction error at each time step $t$, $e_{\text{predict}}(t)$ is defined as 
\begin{align}\label{error_dist}
e_{\text{predict}}(t) = \|\text{dist}_{pi}(t)-\text{dist}_{pj}(t)\|_2,
\end{align}
where $\text{dist}_{pi}$ is the distance between vehicle $i$ and vehicle $j$ predicted by vehicle $i$ (distance from the point of view of vehicle $i$) and, similarly, $\text{dist}_{pj}$ is the distance between vehicle $i$ and vehicle $j$ predicted by vehicle $j$ (distance from the point of view of vehicle $j$). The predicted distances are equivalent to
\begin{equation}\label{error_traj}
\begin{aligned}
\text{dist}_{pi}(t) &\simeq \|\boldsymbol{\tau}^i_{pi}(t) - {\boldsymbol{\bar \tau}}^j_{pi}(t-1)\|_2,\\
\text{dist}_{pj}(t) &\simeq \|\boldsymbol{\tau}^j_{pj}(t) - {\boldsymbol{\bar \tau}}^i_{pj}(t-1)\|_2,
\end{aligned}
\end{equation}
and by substituting \eqref{error_traj} in \eqref{error_dist}, the predicted error is equivalent to 
\begin{equation}
\begin{aligned}
&e_{\text{predict}}(t) \simeq\\
     & \|\bigg(\|\boldsymbol{\tau}^i_{pi}(t) - {\boldsymbol{\bar \tau}}^j_{pi}(t-1)\|_2 - \|\boldsymbol{ \tau}^j_{pj}(t) - {\boldsymbol{\bar \tau}}^i_{pj}(t-1)\|_2\bigg)\|_2.
     \end{aligned}
\end{equation}
Since the cars are rigid bodies (modeled as polytopic sets) and not just point masses, we consider the exact minimum distance between the two polytopic sets and define $\text{dist}_{pi}$ and $\text{dist}_{pj}$ using the notion of distance between the sets. As discussed earlier, the distance between the two polytopic sets $i$ and $j$ is defined as $-{\mathbf{b}^{i}}^{\top} \boldsymbol{\lambda}_{ij} - {\mathbf{b}^{j}}^{\top}\boldsymbol{\lambda}_{ji}$. However, this value is different from the view of vehicle $i$ and vehicle $j$, in distributed approach ($\text{dist}_{pi}\neq \text{dist}_{pj}$). According to distance constraint \eqref{NMPC_dmin}, we have  
\begin{equation}\label{dist_pi}
    \text{dist}_{pi}(t) = -{\mathbf{b}^{i}}(t)^{\top} \boldsymbol{\bar \lambda}_{ij}(t-1) - {\mathbf{\bar b}^{j}}(t-1)^{\top}\boldsymbol{\bar \lambda}_{ji}(t-1),
\end{equation}
\begin{equation}\label{dist_pj}
    \text{dist}_{pj}(t) = -{\mathbf{\bar b}^{i}}(t-1)^{\top} \boldsymbol{\bar \lambda}_{ij}(t-1) - {\mathbf{ b}^{j}}(t)^{\top}\boldsymbol{\bar \lambda}_{ji}(t-1)
\end{equation}
By substituting \eqref{dist_pi} and \eqref{dist_pj} in \eqref{error_dist}, the prediction error $e_{\text{predict}}$ can be computed. After this quantification, we establish an upper-bound on the prediction error. Note that in the centralized approach, the prediction error $e_{\text{predict}}$ is zero since no communication is involved (the approach does not rely on the open-loop trajectory predictions of other vehicles) and $\text{dist}_{pi} = \text{dist}_{pj}$.     
\begin{theorem}
Let the minimum distance between vehicle $i$ and $j$ from the perspective of vehicle $i$ and $j$ be defined according to \eqref{dist_pi} and \eqref{dist_pj}, respectively. By using Algorithm 1 to solve Problem \eqref{eq:MPC_optimization}, the prediction error is bounded, that is,

\begin{equation} \label{upper_bound}
\begin{aligned}
e_{\textrm{predict}}(t) &=\|\textrm{dist}_{pi}(t)-\textrm{dist}_{pj}(t)\|_2\\
    & \leq c_i ||\mathbf{ b}^i(\mathbf{ z}^i(t))-\bar{\mathbf{b}}^i(\bar{\mathbf{z}}^i(t-1))||_2\\
    &+ c_j ||\mathbf{ b}^j(\mathbf{ z}^j(t))- \mathbf{\bar b}^j(\mathbf{\bar z}^j(t-1))||_2,
\end{aligned}
\end{equation}
\end{theorem}
where $c_i$ and $c_j$ are constant scalars. For vehicle applications with rectangular polytopic shapes $c_i$ and $c_j$ are equal to one. For general polytopic shapes $c_i = \sqrt{2}\|({\mathbf{A}_O}^{i{\top}})^{\dagger}\|_{\mathbf{F}} = \sqrt{2\sum_{i=1}^{r} \sigma_{i}^2}$, where $\sigma_i$ is the $i$th singular value of the matrix and $r$ is its rank. Similarly, $c_j$ has the same definition associated with matrix $(\mathbf{A}_O^{j{\top}})^{\dagger}$. 

\begin{proof}
See Appendix.
\end{proof}


\begin{figure}
\centering
\includegraphics[width=0.9 \linewidth]{pics/scenario_example.PNG}
\caption{Overtaking maneuver: the top arrow indicates direction of motion.}
\label{fig:scenario_example}
\end{figure}

To clarify the meaning of this time-varying upper-bound (right-hand side of \eqref{upper_bound}), the overtaking scenario in \figref{fig:scenario_example} is simulated and the minimum distances between the cars at each time step along the simulation is shown in \figref{fig:e_pred_comparison} top plot. As seen in the top plot, $\text{dist}_{pi}$, the distance predicted by car $i$ (light blue line) is different from $\text{dist}_{pj}$, the distance predicted by car $j$  (pink line). The true distance is the actual distance between the cars (gray line). This difference in predicted distances is the prediction error which is bounded according to \eqref{upper_bound}. The bottom plot in \figref{fig:e_pred_comparison}, shows that for overtaking scenario the prediction error $e_{\text{predict}}$ (blue line) is bounded by the computed proposed upper bound (right-hand side of \eqref{upper_bound}) (red line). This upper bound means the prediction error in computing the distance between two cars is bounded by the deviation of the $\mathbf{b}^i$ and $\mathbf{b}^j$ vectors, between two iterations of the distributed algorithm. The distance in dual formulation is proportional to $\mathbf{b}^i$ and $\mathbf{b}^j$, which are right-hand side of polytopic set representation, as shown \figref{fig:geometric_rep}. The error is bounded and it is small, since the vector $\mathbf{b}$ does not change dramatically between two problem iterations.        
\begin{figure}
\centering
\includegraphics[width=\linewidth]{pics/e_pred1.eps}
\caption{\textbf{Top} In distributed approach, the distance between vehicle $i$ and vehicle $j$ from the view of both vehicles is not the same. \textbf{Bottom} The proposed upper-bound of \eqref{upper_bound} is illustrated in red for the overtaking simulation and the prediction error on distance is bounded by the proposed upper-bound.}
\label{fig:e_pred_comparison}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\linewidth]{pics/trivial_bound_comparison.eps}
\caption{The trivial upper-bound is compared versus the proposed upper-bound on distance error.} 
\label{fig:trivial_bound}
\end{figure}

In the remainder of this section, we will address the following questions: \begin{enumerate}
    \item How tight is this bound compared to a trivial upper bound (computed from boundaries of the feasible set)?
    \item For a given acceptable error on the states, how one can rewrite the upper-bound as a function of acceptable error on the states and enforce it as a constraint in NMPC problem \eqref{eq:MPC_optimization}?
    \item How can one normalize the upper-bound values?
\end{enumerate} 

1) To study how tight the upper-bound \eqref{upper_bound} is, we have compared it with a trivial upper-bound. The trivial upper-bound is defined by maximizing the right-hand-side of \eqref{upper_bound}. This maximization is done by substituting maximum boundary values of the feasible set $\mathcal{Z}$ in \eqref{dist_pi} and \eqref{dist_pj}. The results for the same overtaking simulation is shown in \figref{fig:trivial_bound}. The top plot shows that prediction error is bounded by the proposed upper-bound. The bottom plot shows that the proposed upper-bound is considerably tighter than the trivial upper-bound.  

2) For a given acceptable error on the states, we can define a threshold for the upper-bound and include the upper-bound \eqref{upper_bound} in the NMPC formulation \eqref{eq:MPC_optimization} to bound the prediction error in the distributed problem. For our application, the states are $x$,$y$ and $\psi$. The maximum error on $x$, $y$ and $\psi$ are denoted as $e_x$, $e_y$ and $e_{\psi}$, respectively and defined as  
\begin{equation}\label{error_eq}
\begin{aligned}
    e_x &= |x(t) - \bar{x}(t-1)|\\
    e_y &= |y(t) - \bar{y}(t-1)|\\
    e_{\psi} &= |\psi(t) - \bar{\psi}(t-1)|
\end{aligned}
\end{equation}

\begin{corollary}
Given the acceptable error values on the states $e_x$, $e_y$ and $e_{\psi}$, let $e_x$, $e_y$ and $e_{\psi}$ be defined as \eqref{error_eq}, one can compute $\alpha_{\text{min}}\geq 0$, such that the following holds for all $t\geq 0$:
\begin{equation}\label{threshold}
||\mathbf{ b}^i(\mathbf{z}^i(t))-\bar{\mathbf{b}}^i(\bar{\mathbf{z}}^i(t-1))||_2 \leq \alpha_{\text{min}}(t).  
\end{equation} 
Then by enforcing \eqref{threshold} as a constraint in the NMPC problem \eqref{eq:MPC_optimization}, if the problem \eqref{eq:MPC_optimization} is feasible, the prediction error for each state will not violate the acceptable specified error.  
\end{corollary}
\begin{proof}
To quantify the equation \eqref{upper_bound} based on acceptable error we have
\begin{equation}\label{upper_bound_threshold}
\begin{aligned}
&||\mathbf{ b}^i(\mathbf{ z}^i(t))-\bar{\mathbf{b}}^i(\bar{\mathbf{z}}^i(t-1))||_2\\
=& ||\mathbf{A}(\psi(t))\begin{bmatrix}
x(t)\\
y(t)
\end{bmatrix}-\mathbf{A}(\bar{\psi}(t-1))\begin{bmatrix}
\bar{x}(t-1)\\
\bar{y}(t-1)
\end{bmatrix}||_2\\
=&||\mathbf{A}(\bar{\psi}(t-1) \pm e_{\psi})\begin{bmatrix}
\bar{x}(t-1) \pm e_x\\
\bar{y}(t-1) \pm e_y
\end{bmatrix}\\
&-\mathbf{A}(\bar{\psi}(t-1))\begin{bmatrix}
\bar{x}(t-1)\\
\bar{y}(t-1)
\end{bmatrix}||_2 = \alpha(t).
\end{aligned}
\end{equation}
We minimize the right-hand side of \eqref{upper_bound_threshold} (all the values are known but different combinations of signs must be considered to find the minimum $\alpha(t)$), then we compare the upper-bound with the threshold value $\alpha_{\text{min}}(t)$ 
\end{proof}
%The prediction error in distributed algorithm leads to an acceptable level of suboptimality while the inequality \eqref{threshold} is satisfied, otherwise the algorithm does not respect the specified prediction error limits.
3) To correlate the upper-bound values with specified acceptable predicted error, the upper-bound is normalized by $\alpha_{\text{min}}(t)$. For the overtaking simulation scenario, the acceptable errors are specified as $e_x = 1$, $e_y = 0.5$, and $e_{\psi} = 0.2$ and $\alpha_{\text{min}}(t)$ is computed from \eqref{upper_bound_threshold} and then the upper-bound is normalized by $\alpha_{\text{min}}$, this normalization ratio $\frac{||\mathbf{ b}^i(\mathbf{z}^i(t))-\bar{\mathbf{b}}^i(\bar{\mathbf{z}}^i(t-1))||}{\alpha_{\text{min}}}$ is shown in \figref{fig:alpha_ratio}. The prediction error increases as the ratio gets closer to one and decreases as the ratio gets closer to zero. This ratio can be penalized in the cost function in \eqref{eq:MPC_optimization} to keep the prediction error close to the acceptable range specified by design engineer.  

\begin{figure}
\centering
\includegraphics[width=\linewidth]{pics/alpha_ratio.png}
\caption{The ratio of upper-bound with respect to $\alpha$ is shown.} 
\label{fig:alpha_ratio}
\end{figure}




 






